Online Energy Minimization Under A Peak Age of Information Constraint

We consider a node where packets of fixed size (in bits) are generated at arbitrary intervals. The node is required to maintain the peak age of information (AoI) at the monitor below a threshold by transmitting potentially a subset of the generated packets. At any time, depending on the packet availability and the current AoI, the node can choose which packet to transmit, and at what transmission speed (in bits per second). Power consumption is a monotonically increasing convex function of the transmission speed. In this paper, for any given time horizon, the objective is to find a causal policy that minimizes the total energy consumption while satisfying the peak AoI constraint. We consider competitive ratio as the performance metric, that is defined as the ratio of the expected cost of a causal policy, and the expected cost of an optimal offline policy that knows the input (packet generation times) in advance. We first derive a lower bound on the competitive ratio of all causal policies, in terms of the system parameters (such as power function, packet size and peak AoI threshold), and then propose a particular policy for which we show that its competitive ratio has similar order of dependence on the system parameters as the derived lower bound.

==> MaxSpeedLess.tex <==
\section{Maximum transmission speed $s^{\max}\le 2W/D$} \label{appendix:smax<2W/D}
\begin{remark} \label{remark:d(0)>T}
	Note that if the initial deadline $d(0)>T$, then an optimal causal/offline policy should not transmit any packet (constraints \eqref{eq:p-deadline-constraint} and \eqref{eq:p-speed-constraint} are automatically satisfied, and energy consumption is $0$). Hence, for the rest of the analysis, we only consider the non-trivial setting where $d(0)\le T$, and any policy that satisfies the deadline constraint \eqref{eq:p-deadline-constraint} must transmit at least one packet completely until time $d(0)$.
\end{remark}

For an offline policy $\pi$ that satisfies the deadline constraint \eqref{eq:p-deadline-constraint}, we showed in the proof of Lemma \ref{lemma:2W-per-D} that if $\pi$ completely transmits a packet $i$ generated at time $g_i<T-D$, then in interval $[g_i,g_i+D)$ (which is of length $D$ time units), $\pi$ transmits at least two packets ($2W$ bits) completely (packet $i$ followed by a newer packet). $(i)$ When $s^{\max}=2W/D$, this is possible only if $\pi$ transmits packet $i$ at constant speed $s^{\max}=2W/D$ over the interval $[g_i,g_i+D/2)$, and a newer packet at constant speed $s^{\max}=2W/D$ over the interval $[g_i+D/2,g_i+D)$. $(ii)$ When $s^{\max}<2W/D$, policy $\pi$ can never transmit $2W$ bits in interval $[g_i,g_i+D)$, which implies that $\pi$ completely transmits a packet $i$ only if its generation time $g_i>T-D$. 
Hence, we have the following result.
\begin{lemma} \label{lemma:g_i>T-D}
	Consider an offline policy $\pi$ that satisfies constraints \eqref{eq:p-deadline-constraint} and \eqref{eq:p-speed-constraint}. For any packet generation sequence $\sigma\in\Sigma(s^{\max})$: $(i)$ If $s^{\max}=2W/D$, then for any packet $i$ that $\pi$ transmits completely, if the generation time $g_i\le T-D$, then $\pi$ transmits packet $i$ at a constant speed $2W/D$, over the interval $[g_i,g_i+D/2)$, followed by the transmission of a newer packet at constant speed $s^{\max}=2W/D$ over the interval $[g_i+D/2,g_i+D)$. $(ii)$ If $s^{\max}<2W/D$, then $\pi$ completely transmits a packet $i$, only if its generation time $g_i>T-D$. 
\end{lemma} 

\subsubsection{$s^{\max}=2W/D$}
From Lemma \ref{lemma:g_i>T-D}, we know that if an offline policy has to completely transmit a packet $i$ with generation time $g_i\le T-D$, then it transmits it with constant speed $s^{\max}=2W/D$ over the interval $[g_i,g_i+D/2)$, followed by the transmission of a newly generated packet $j$ at constant speed $2W/D$ over the interval $[g_i+D/2,g_i+D)$. Note that if generation time of update $j$ is $g_j\le T-D$, by from Lemma \ref{lemma:g_i>T-D} it again follows that $g_j=g_i+D/2$ (transmission of packet $j$ starts at its generation time). Hence, we have the following two sub-cases:
\paragraph{$\pi$ completely transmits an update $i$ generated at time $g_i\le T-D$} In this case, $\pi$ completely transmits a sequence of updates generated at time $g_i,g_i+D/2,g_i+D,g_i+3D/2,\cdots,g_i+aD/2$, where $a$ is the smallest positive integer such that $g_i+aD/2>T-D$. Note that this is possible only if packets are generated at these time instants, thus partially characterizing the set of packet generation sequences $\Sigma(s^{\max}=2W/D)$ for which the constraints \eqref{eq:p-deadline-constraint} and \eqref{eq:p-speed-constraint} can be satisfied. 

\paragraph{$\pi$ does not transmit any update $i$ with $g_i\le T-D$, completely} 

\subsubsection{$s^{\max}<2W/D$}
From Lemma \ref{lemma:g_i>T-D}, we know that when $s^{\max}<2W/D$, an offline policy $\pi$ completely transmits a packet $i$ only if its generation time is $g_i>T-D$.
Note that if policy $\pi$ completes transmitting a packet $i$ (with generation time $g_i>T-D$), at time $\tau_i>g_i$, then at any time $t\in[\tau_i,T]$, the deadline $d(t)=g_i+D>T\ge t$. Hence, once a packet $i$ ($g_i>T-D$) gets completely transmitted, an optimal offline policy $\pi^\star$ (that consumes minimum energy and satisfies constraints \eqref{eq:p-deadline-constraint} and \eqref{eq:p-speed-constraint}), should not transmit any other packet. This fact together with Remark \ref{remark:d(0)>T} and Lemma \ref{lemma:g_i>T-D} implies that $\pi^\star$ completely transmits exactly one packet $i^\star$. Also, the generation time of $i^\star$ is $g_{i^\star}>T-D$, and transmission completion time is $\tau_{i^\star}<d(0)$. Since the power function $P(\cdot)$ is increasing, we get the following result.
\begin{lemma} \label{lemma:opt-offline}
	For $s^{\max}<2W/D$ and packet generation sequences $\sigma\in\Sigma(s^{\max})$, an optimal offline policy $\pi^\star$ completely transmits exactly one packet $i^{\star}=\arg\min_{i}\{g_i|g_i>T-D\}$, with 	constant speed $W/(d(0)-g_{i^\star})$ over the interval $[g_{i^\star},d(0))$. 
\end{lemma}  

Note that the optimal offline policy $\pi^\star$ characterized in Lemma \ref{lemma:opt-offline} is essentially a threshold policy that can be implemented using only causal information: idle until a packet $i$ is generated with generation time $g_i>T-D$, and then begin to transmit packet $i$ (immediately) at constant speed $W/(d(0)-g_i)$ until completion, and then again idle indefinitely. Hence, for the specific case when $s^{\max}<2W/D$, we have a causal threshold policy with competitive ratio $1$ (over the set of packet generation sequences $\Sigma(s^{\max})$.
\begin{lemma}
	Optimal offline policy $\pi^\star$ characterized in Lemma \ref{lemma:opt-offline} is an optimal causal policy with competitive ratio $1$.
\end{lemma}

%	As shown in Lemma \ref{lemma:2W-per-D}, in interval $[t_i,t_i+D)$ (of length $D$), $\pi$ must transmit at least $2W$ bits completely. However, this is not possible since $\pi$ transmits at speed less than $2W/D$ (speed constraint \eqref{eq:p-speed-constraint}).Hence, $\pi$ cannot satisfy constraints \eqref{eq:p-speed-constraint} and \eqref{eq:p-deadline-constraint} simultaneously.
%\end{IEEEproof}


==> proof_lemma_pi_p_feasible.tex <==
As shown in Lemma \ref{lemma:2W-per-D}, if a policy $\pi$ completely transmits a packet $i$ generated at time $t_i$, then the new deadline will be $t_i+D$. If $t_i+D<T$, then to satisfy the deadline constraint \eqref{eq:p-deadline-constraint}, $\pi$ should completely transmit another packet $j$ (generated at time $t_j>t_i$) before $t_i+D$. However, this is possible only if $(i)$ the maximum speed at which the policy can transmit is $s^{\max}\ge 2W/D$, and $(ii)$ $t_j\le (t_i+D)-W/s^{\max}$ (i.e., the inter-generation time of packets is at most $D-W/s^{\max}$). Therefore, to prove Lemma \ref{lemma:pi-p-feasible}, without loss of generality, we let $s^{\max}\in[2W/D,3W/D)$, and inter-generation time of packets less than $D-W/s^{\max}$.

Consider the set of packets $\cI$ that $\pi^p$ transmits completely. %Since $\pi^p$ transmits a packet over contiguous interval (an interrupted packet is never transmitted again), 
$\cI$ can be partitioned into subsets $\cI_p$ and $\cI_s$, where $\cI_p$ denotes the set of completely transmitted packets that $\pi^p$ begins to transmit immediately after generation, while $\cI_s$ is the set of completely transmitted packets that $\pi^p$ does not begin to transmit at generation. 
Note that $\pi^p$ never idles when there is a fresh packet to transmit. Also, $\pi^p$ interrupts the packet under transmission at time $t$ only if %a new packet is generated at time $t$ that 
it can completely transmit the newly generated packet until time $d(t)$ (i.e. if $d(t)-t\ge W/s^{\max}$). Therefore, if any policy can completely transmit a packet before the initial deadline $d(0)$, then $\pi^p$ also completely transmits some packet before $d(0)$. Furt, 

 shows that any policy $\pi$ that satisfies the deadline constraint \eqref{eq:p-deadline-constraint}, if completely transmits a packet generated at time $t$, then transmits at least two complete packets (i.e. $2W$ bits) in interval $[t,t+D)$ (assuming $t+D<T$). However, this is possible only if in interval $[t,t+D)$, $\pi$ transmits at an average (maximum) speed at least $2W/D$. Therefore, any policy $\pi$ may satisfy both constraints \eqref{eq:p-deadline-constraint} and \eqref{eq:p-speed-constraint} simultaneously, only if $s^{\max}\ge 2W/D$. Hence, to prove Lemma \ref{lemma:pi-p-feasible}, it is sufficient to consider the case where $s^{\max}\in[2W/D,3W/D)$. Moreover, since a feasible policy can transmit a packet at maxi
%\begin{align} \label{eq:smax-bet-2to3}
%	s^{\max}\in[2W/D,3W/D).
%\end{align}


Note that $\pi^p$ never idles if there is a fresh packet to transmit.
